A machine learning approach for efficient uncertainty quantification using multiscale methods

Several multiscale methods account for sub-grid scale features using coarse scale basis functions. For example, in the Multiscale Finite Volume method the coarse scale basis functions are obtained by solving a set of local problems over dual-grid cells. We introduce a data-driven approach for the estimation of these coarse scale basis functions. Specifically, we employ a neural network predictor fitted using a set of solution samples from which it learns to generate subsequent basis functions at a lower computational cost than solving the local problems. The computational advantage of this approach is realized for uncertainty quantification tasks where a large number of realizations has to be evaluated. We attribute the ability to learn these basis functions to the modularity of the local problems and the redundancy of the permeability patches between samples. The proposed method is evaluated on elliptic problems yielding very promising results.

==> _region_.tex <==
\message{ !name(methodology.tex)}
\message{ !name(methodology.tex) !offset(-2) }
\section{Methodology}
We consider the task of solving equations~\eqref{eq:pressure} and
\eqref{eq:saturation} on 1000 isotropic permeability fields for the
purpose of uncertainty quantification. In all cases, water is injected
into a reservoir initially containing only oil. The domain is the unit
square $[0,1]^2\subset \mathbb{R}^2$ discretized by a $81\times81$
Cartesian grid. The (primal) coarse partition for the MSFV method is
chosen as a $9\times9$ coarse Cartesian grid. The log-permeability
field realizations are generated assuming a zero mean gaussian random
field with exponential covariance
$$\operatorname{Cov}(\mathbf r_1, \mathbf r_2) = \sigma^2\exp\left(-\frac{\lVert
    \mathbf r_1-\mathbf r_2 \rVert}{L}\right)$$ where we choose
$L=0.1$
as the correlation length, and $\sigma=1.0$
as the standard deviation of the random field. \textbf{ADD EXAMPLE OF PERM FIELD...}

Before we continue, we need to introduce some terminology. We define
\emph{interior} basis functions as those basis functions whose support
regions do \emph{not} touch the domain boundary. For example, our
coarse partition of $9\times 9$ contains $7\times 7 = 49$ interior
basis functions. For practical purposes, we shall limit ourselves to
interior basis functions, i.e. we build a surrogate to generate
interior basis functions while letting the remaining basis functions
be computed normally with the system of equations~\eqref{eq:local_prob}.

We define a \emph{permeability patch} as the cropped region of the 2D
permeability field that corresponds to the support region of a basis
function. In the learning framework, the permeability patches
$\kappa^1, \kappa^2, \cdots, \kappa^N$ are our inputs, and the
corresponding basis functions $\phi^1, \phi^2, \cdots, \phi^N$ are our
outputs.  For our configuration, the array size of each output basis
function is $19\times 19$, and the array size of each input
permeability patch is $19\times 19 \times d$, where $d=1$ for
isotropic fields, and $d=2$ in the anisotropic case.

The method we propose consists on training a neural network surrogate
with a dataset of 1000 samples
$\{(\kappa^1,\phi^1),\cdots,(\kappa^{1000},\phi^{1000})\}$. This
amounts to a little over 20 full MSFV simulation runs (since each run
yields 49 samples). Once the network is trained, we use it to
solve~\eqref{eq:pressure} and \eqref{eq:saturation} on 1000
realizations of the permeability field $\mathbf{K_1}, \mathbf{K_2},
\cdots, \mathbf{K_{1000}}$. We then perform statistics on some
quantities of interest, e.g. pressure at a given point, production
curves, water breakthrough time, etc.

\textbf{ADD A WORKFLOW CHART...}.

\subsection{Architecture and optimization}
The architecture employed is a 1-hidden layer with ReLU
activation. The size of the hidden layer is determined via validation
from a finite set of options, namely $\{64, 128, 256, 512,
1024\}$. Naturally, the input and output layers are of size
$19\times19=361$, matching the size of the permeability patches
(isotropic case) and basis functions.

One property of the basis functions is that they take values between
0 and 1. To embed this information into the network, we use a
\emph{hard sigmoid} as the output activation instead of the usual
linear activation employed in regression tasks. The hard sigmoid is
defined as the function
${x\in\mathbb{R} \mapsto \max(0,\min(1,0.2x+0.5))}$.

For the regularization, we use dropout after the hidden layer, plus $L^1$
and $L^2$ norm penalties for the weights of the hidden layer. The
values for these are tuned via validation.

For the optimization, we employ the gradient-based algorithm
Adam. Again, the learning rate is tuned via validation. We choose to
compute the gradient at each iteration using the whole training set
(as opposed to mini-batch gradient descent) since the set is small.

We see that there are many hyperparameters to be adjusted (layer size,
coefficients for the $L^1$ and $L^2$ penalties, dropout percentage,
learning rate). We use the Python package \texttt{hyperopt} to perform
the hyperparameter optimization. For the validation set, we randomly
set aside 200 samples (20\%) from the dataset.

\subsection{Post-processing: ensuring partition of unity}
A set of basis functions in a given function space must conform a
partition of unity. Such requirement is not necessarily fulfilled in
the learning model. A post-processing of the basis functions has to be
performed to ensure this property. Let
$\{\phi^1, \phi^2, \cdots, \phi^{N_C}\}$ be the set of pre-processed
basis functions, then the new basis functions are defined as
$$\phi^i_{new}(x) = \frac{\phi^i(x)}{\sum_k \phi^k(x)}$$
In effect, big improvements have been seen after performing this
post-processing step.

\message{ !name(methodology.tex) !offset(-92) }


==> notes.tex <==
reviewer 1

1. Any ML technique can be used. We explored LR. We found NN works better because ...

3. GPs, bagging in NN, NN with dropout for predictor uncertainty, neglecting did not affect results

2. how did we actually come up with the arch

reviewer 2

1. provide time estimate, major advances in NN opt to make it useful in practice... GPUs etc
2. In ms methods we do not need to use coarse grids with different coarse cell sizes as the subscale is captured by the bfs.
about the msfem: it does not scale with N, does not exploit spatial redundancy within a single realization 

